Distributed Work Stealing in a Task-Based Dataflow Runtime

The task-based dataflow programming model has emerged as an alternative to the process-centric programming model for extreme-scale applications. However, load balancing is still a challenge in task-based dataflow runtimes. In this paper, we present extensions to the PaR-SEC runtime to demonstrate that distributed work stealing is an effective load-balancing method for task-based dataflow runtimes. In contrast to shared-memory work stealing, we find that each process should consider future tasks and the expected waiting time for execution when determining whether to steal. We demonstrate the effectiveness of the proposed work-stealing policies for a sparse Cholesky factorization, which shows a speedup of up to 35% compared to a static division of work.

==> paper/dataflow.tex <==
\section{Dataflow Programming Model}
\label{section: dataflow}

% WHAT IS DATAFLOW PROGRAMMING MODEL? HOW IS IT DIFFERNT FROM OTHER TASKBASED MODELS?

A dataflow programming model \cite{KARP1969147} allows the movement of data from one task to another and the execution of an application is progressed along this flow of data. In this model, a task is said to be \textit{ready} when all its input data become available locally. Due to the inherent parent-child relation introduced amongst the tasks, by the data flow, the entire program in a dataflow programming model can be modelled as a directed acyclic graph (DAG), D = (V,E). Each vertex, $v \in V$, represents a task and each edge, $(v_i,v_j) \in E$, represents parent-child relation between two vertices (tasks). Potentially parallel sections are easily identified from the DAG, which makes the dataflow programming model more asynchronous when compared to the traditional control-flow programming model. 

\subsection{PaRSEC }
\input{paper/parsec}

\subsection{Templated Task Graph (TTG)}
\input{paper/ttg}


==> paper/experiment/observation.tex <==
\subsection{Main Observations}

The main observations from the experiments carried out are as follows:
\begin{enumerate}
    \item Work stealing is effective only when there is significant work imbalance.
    \item Counting future tasks when determining starvation has a significant effect on work stealing.
    \item The best-performing victim policy considers task waiting time.
    \item Work stealing reduces variations in execution time.
    \item Successful steals do not guarantee speedup.
\end{enumerate}

==> paper/experiment/scheduler.tex <==
\subsection{Scheduling Policy}


%\begin{figure}[h]
%  \centering
%  \includegraphics[width=\linewidth]{images/scheduler_4Node_exectime.png}
%  \caption{Execution time for different victim policy for Two\_Queue scheduler and AP scheduler.}
%  \small
%  \label{fig: scheduler_4Node_exectime}
%\end{figure}


% LaTeX evil: if I take this duplicate figure out, it doesn't print!
%\begin{figure}[htbp]
%  \centering
%  \includegraphics[width=.5\textwidth]{images/scheduler_4Node_exectime_half.png}
%  \caption{Execution time when using \textit{Half} for 2Q scheduler and AP scheduler.\\Experiment conducted on four nodes using a 10000x10000 double precision tiled matrix where each tile has a size of 50x50.}
%  \label{fig: scheduler_4Node_exectime_half}
%\end{figure}


Two metrics were used to compare the effectiveness of the two scheduling policies 2Q and AP for work stealing: the percentage of tasks rescheduled out of all scheduled tasks and the average task stolen per successful steal.
A scheduling policy is effective for work stealing if the former metric is low and the latter metric is high.
Our experiments demonstrate that the 2Q is more effective for work stealing as compared to the AP.
Table~\ref{table: scheduler_effectiveness} shows the percentage of tasks rescheduled for different victim policies when using AP.
The rescheduling problem is the worst for \textit{Half} and comparatively limited for \textit{Single} and \textit{Chunk}.
Fig.~\ref{fig: scheduler_4Node_exectime_half} also demonstrates that high rescheduling rate in \textit{Half} also affects the performance of work stealing.
Table~\ref{table: scheduler_effectiveness} gives the average task stolen per steal request with different scheduling policies for different victim policies.
Higher rates of average task stolen per steal imply better task discovery.
From Table~\ref{table: scheduler_effectiveness} it is observable that task discovery is better with the 2Q. All the experiments show that 2Q is a better scheduling policy for work stealing when compared to AP. 


\begin{figure}[htbp]
  \centering
  \includegraphics[width=.5\textwidth]{images/scheduler_4Node_exectime_half.png}
  \caption{Execution time when using \textit{Half} for 2Q scheduler and AP scheduler. Global matrix of $10000^2$ 64-bit elements, organized as $200^2$ tiles of $50^2$ elements}
  \label{fig: scheduler_4Node_exectime_half}
\end{figure}


\begin{table}[htbp]
\centering
\caption{Effectiveness of scheduling policy 2Q and AP with respect to work stealing.}
\label{table: scheduler_effectiveness}
\begin{tabular}{l|rrr}
\toprule
& \textbf{Single} & \textbf{Chunk} & \textbf{Half} \\
\midrule
\textbf{\% of rescheduled tasks with AP}                   & 0.08                                & 1.51                                & 99.14                               \\
\textbf{Avg tasks stolen per successful steal with AP} & 0.68                                & 1.69                               & 12.26                              \\
\textbf{Avg tasks stolen per successful steal with 2Q} & 0.90                                 & 16.07                              & 247.29                             \\
\bottomrule
\end{tabular}
\end{table}




==> paper/parsec.tex <==
\begin{figure}[h]
  \centering
     \input{images/layout}
  \caption{PaRSEC Layout}
  \label{fig: parsec_layout}
\end{figure}


 PaRSEC is a task-based dataflow runtime, where the execution of tasks is fully distributed with no centralized components.
 The PaRSEC framework consists of three layers as shown in Fig.~\ref{fig: parsec_layout}. The bottom layer (hardware layer) interacts with different computing resources while the middle layer (parallel runtime layer) abstracts these computing resources to the application developer. Task scheduling, detecting local and remote dependencies, data movement between nodes, and distributed termination detection \cite{bosilca2020} are all the responsibility of the middle layer. The top layer (domain specific language layer) contains the domain-specific languages~\cite{Hoque2017a,Bosilca2020TheTT} that PaRSEC provides for developers to express their applications. The user is responsible for defining the tasks and the dependencies amongst the tasks using these domain-specific languages. The user also defines how the tasks are mapped to different computing nodes.
 PaRSEC uses MPI for communication between nodes.
 

%The PaRSEC runtime is divided into five modules - communication module, scheduler module, dependency management module, data management module and termination detection module. 

%\textbf{Scheduler Module}: The scheduler module selects a \textit{ready} task, from a list of ready tasks for execution. A task is in \textit{ready} state if all its data items are available locally. %In PaRSEC each worker thread runs a copy of the scheduler. 

%\textbf{Data Management Module}: Whenever a task execution is completed, it generates data items that are used by its successor tasks. This module is responsible for the storage of these data items in such a way that all the successors of a task can find the required data items. 

%\textbf{Communication Module}: A separate thread, called the communication thread, is used for all data movements in PaRSEC. When a task execution is completed by a worker thread and if this particular task has remote successors (successor task mapped to another node), the worker thread transfers the details of the data item to the communication thread. The communication thread then sends a message to the remote node with details of the data item. When this message is received by the communication thread in the receiver node, the information in the message is used to initiate a handshake that will fetch the data item from the sender node.

%\textbf{Dependency Management Module}: The dependencies of every task is managed by the dependency management module. When the data fetch handshake is complete and the data items are received by a node, the data items are marked as available for all the tasks that depend on it.  When all the data items required for a task become available the task is deemed ready for execution.

%\textbf{Termination Detection Module}: PaRSEC uses the \textit{4 counter wave}  algorithm in \cite{bosilca2020} to detect distributed termination. 

\subsubsection{Domain Specific Languages (DSL)}

In PaRSEC, each task is an instance of a \textit{Task Class} which defines task actions and properties.
The only difference between tasks of the same task class is the unique key that identifies each task and the data items on which the task operates.
For example, PaRSEC program for Cholesky factorization of a tiled matrix will have only four task classes---\texttt{potrf}, \texttt{trsm}, \texttt{syrk}, and \texttt{gemm}---irrespective of the the number of tiles in the matrix. On the other hand, the number of tasks belonging to these task classes will differ according to number of tiles. A DSL in PaRSEC helps the user define the different task classes in a program. At present, there are three DSLs available in PaRSEC:  Parameterized Task Graph (PTG) \cite{Hoque2017a},  Dynamic Task Discovery (DTD) \cite{Bosilca2012}, and Templated Task Graph (TTG) \cite{Bosilca2020TheTT}.
In this paper, we focus on TTG, as it can better handle irregular workloads when compared to PTG and DTD, but the principles we present are applicable to any PaRSEC DSL.

